The Markovianity of Time: The Category Mistake in Open Quantum Systems

The Markov approximation is arguably the most ubiquitous tool in physics, underpinning quantum master equations, stochastic processes, and -- via Shannon's channel model and Lamport's logical clocks -- the foundational assumptions of distributed computing. It is widely assumed that Markovianity inherently implies temporal asymmetry: that the Markov property is a forward-in-time-only (FITO) construct. We show that this assumption is a category mistake in the sense of Ryle (1949). Guff, Shastry, and Rocco (2025) have recently demonstrated that the Markov approximation applied to the Caldeira-Leggett model -- a paradigmatic open quantum system -- maintains time-reversal symmetry in the derived equations of motion. The resulting time-symmetric formulations of quantum Brownian motion, Lindblad master equations, and Pauli master equations describe thermalisation that can occur in two opposing temporal directions. Asymmetry arises not from the dynamics but from boundary conditions. We trace how Markovianity's assumed directionality propagated from physics through Shannon's information theory to Lamport's happens-before relation and the impossibility theorems of distributed computing (FLP, CAP, Two Generals). Each step encodes FITO as convention, then treats it as physical law -- the same category mistake repeated across domains. The Surrey result establishes that this conflation is not merely philosophically suspect but mathematically unnecessary: the most fundamental approximation used to derive irreversibility is itself time-symmetric.

==> dae-handout-commands.tex <==
% --- dae_commands.tex ---

% --- FAQ/Answer macros ---
\newcommand{\question}[1]{%
  \stepcounter{qctr}%
  \vspace{5pt}
  \noindent
  \rule{0.5\columnwidth}{0.5pt}\\
  \noindent
  \phantomsection
  \textbf{[Q\decimal{qctr}]}~%
  \def\a##1\par{##1}{#1}%
  \addcontentsline{loq}{section}{Q\protect\numberline{\theqctr}{{#1}}}
}

\newcommand{\answer}{%
  \vspace{5pt}
  \noindent
  \textbf{[A\decimal{qctr}]}
}

\newcommand{\statement}{%
  \vspace{5pt}
  \noindent
  \textbf{[S\decimal{qctr}] Statement: }
}

\newcommand{\insight}{%
  \vspace{5pt}
  \noindent
  \textbf{[A\decimal{qctr}} Insight: ]
}

\newcommand{\sublistofquestions}{%
  \onlyinsubfile{\vspace{0pt} \large \listofquestions \normalsize \medskip}
}

% --- Subfiles helpers ---
\newcommand{\onlyinsubfile}[1]{#1}
\newcommand{\notinsubfile}[1]{}

% --- Insert Hyperlink (file) ---
\newcommand{\ihl}[2]{%
  \vspace{6pt} \noindent [\hyperlink{./Exhibits/#1.pdf.1}{#1}]{ #2}
}

% --- Insert Menu Item (file/comment) ---
\newcommand{\imi}[2]{%
  \vspace{10pt}
  \noindent
  \textbf{\href{run:FAQ-#1.pdf}{#1}}\\{#2}
}

% --- Strikeout Displaystyle ---
\newcommand{\displayst}[1]{\textrm{\st{$\displaystyle#1$}}}

% --- Custom Horizontal Rule ---
\newcommand{\srule}{%
  \vspace{2pt}
  \noindent\rule{\textwidth}{0.8pt}
}

% --- Leibniz Bridge sibling document references ─────────────────
% \daeref{label}{filename}{description}
%   Links to a sibling document in the same project folder.
%   Rendered in linkred. Margin note shows label + description.
%   Auto-detects format from extension and annotates [PDF] or [HTML].
%   Uses \href{run:filename} so macOS opens the right application.
%   In arXiv/HTML mode: becomes a footnote (no margin note).
%
% Usage:
%   \daeref{DAE-TR-0007}{DAE-TR-0007.pdf}{The Category Mistake}
%   \daeref{CAP Paper}{oae-cap-tufte.html}{HTML with responsive sidenotes}
%
\makeatletter
\newcommand{\dae@detectformat}[1]{%
  \dae@checkhtml#1.html\@nil
}
\def\dae@checkhtml#1.html#2\@nil{%
  \def\dae@temp{#2}%
  \ifx\dae@temp\empty
    \def\dae@fmt{PDF}%  no .html found, assume PDF
  \else
    \def\dae@fmt{HTML}%
  \fi
}
\ifarxiv
  \newcommand{\daeref}[3]{%
    \dae@detectformat{#2}%
    \href{#2}{\textcolor{linkred}{#1}}%
    \footnote{\textcolor{linkred}{#1}\enspace[\dae@fmt]\enspace #3}%
  }
\else
  \newcommand{\daeref}[3]{%
    \dae@detectformat{#2}%
    \href{run:#2}{\textcolor{linkred}{#1}}%
    \marginnote{\scriptsize\textcolor{linkred}{#1}\enspace\textsc{[\dae@fmt]}:\enspace #3}%
  }
\fi
\makeatother

% --- Leibniz Bridge Margin TOC (standardized) ---
% Usage: place \daemargintoc after \maketitle / \placebadges on the first page.
% Requires: etoc, hyperref, linkgreen colour defined,
%           Bitstream Charter via mathdesign (provides bold small caps).
% Sections: bold small caps, green, with number.
% Subsections: regular small caps, green, indented.
% Section short titles MUST be in Title Case for the small-caps effect.
% In arXiv/HTML mode: suppressed (arXiv generates its own TOC sidebar).
\newcommand{\daemargintoc}{%
  \ifarxiv\else
  \marginnote{%
    \hypersetup{linkcolor=linkgreen}%
    \small
    \setcounter{tocdepth}{2}%
    \etocsetstyle{section}{}{\par\vspace{1em}\noindent\leftskip=0em%
      \parbox[c]{1.5em}{\centering\etocnumber}%
      \parbox[c]{\dimexpr\marginparwidth-3em\relax}{\linespread{0.75}\selectfont\raggedright\textbf{\textsc{\etocname}}}%
      \hfill\etocpage\par}{}{}%
    \etocsetstyle{subsection}{}{\par\vspace{0.5em}\noindent\leftskip=1.5em%
      \parbox[c]{1.5em}{\centering\etocnumber}%
      \parbox[c]{\dimexpr\marginparwidth-3em\relax}{\linespread{0.75}\selectfont\raggedright\textsc{\etocname}}%
      \hfill\etocpage\par}{}{}%
    \etocsettocstyle{}{}%
    \tableofcontents
  }%
  \fi
}

\NewDocumentCommand{\marginfig}{O{width=\linewidth} m o o o o}{%
  \begin{marginfigure}\IfValueT{#6}{[#6]}%
    \IfValueTF{#5}{#5}{\centering}%
    \includegraphics[#1]{#2}%
    \IfValueTF{#3}{%
      \caption{#3}%
    }{%
      \caption{#2}%
    }
    \IfValueTF{#4}{%
      \label{#4}%
    }{%
      \label{fig:#2}%
    }
  \end{marginfigure}
}

\NewDocumentCommand{\fig}{O{width=\linewidth} m o o}{%
  \begin{figure}
    \centering
    \includegraphics[#1]{#2}% 
    \IfValueTF{#3}{%
      \caption{#3}%
    }{%
      \caption{#2}%
    }
    \IfValueTF{#4}{%
      \label{#4}%
    }{%
      \label{fig:#2}%
    }
  \end{figure}
}


==> dae-handout-settings.tex <==
% Document class

% Core packages
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{microtype}
\usepackage{xparse}
\usepackage{amsmath,amssymb}
\usepackage{graphicx}
\usepackage{xcolor}
\usepackage{booktabs}
\usepackage{lipsum}
\usepackage{epigraph}
\usepackage{framed}
\usepackage{todonotes}
\usepackage[most]{tcolorbox}

% Specialized
\usepackage{tikz}
% \usepackage{bytefield}  % deprecated across all DAE publications
\usepackage{eso-pic}

% Graphics path (Leibniz Bridge convention):
%   ./figures/    — local working copies (populated by pull-figures.sh)
%   ../Figures/   — shared parent folder
%   ../../Figures/ — grandparent
%   FIGURES/      — absolute iCloud master (last resort)
\graphicspath{{./}{./figures/}{../Figures/}{../../Figures/}{./images/}{./graphics/}}

% ── Leibniz Bridge colour scheme ─────────────────────────────────
% Green: internal navigation (same document) — \ref, \cite, TOC
% Blue:  external web links — \url, \href to http(s)
% Red:   sibling documents (PDF, HTML in same project folder)
\definecolor{linkblue}{RGB}{30, 80, 180}
\definecolor{linkgreen}{RGB}{30, 120, 60}
\definecolor{linkred}{HTML}{AE0000}

% Hyperref
\usepackage{hyperref}
\hypersetup{
  colorlinks=true,
  urlcolor=linkblue,          % \url and \href to web
  linkcolor=linkgreen,        % \ref, \eqref, \pageref, TOC
  citecolor=linkgreen,        % \cite (jumps to bib within this doc)
  filecolor=linkred,          % \href{run:...} local file links
}

% Font commands
\newcommand{\headerfont}{\fontfamily{phv}\selectfont}
\newcommand{\titlefont}{\headerfont\Huge\bfseries}
\newcommand{\authorfont}{\headerfont\large}
\newcommand{\datefont}{\headerfont\normalsize}

% Custom title page
\makeatletter
\renewcommand{\maketitle}{
  \newpage
  \thispagestyle{empty}
  \begin{fullwidth}
    \centering
    {\titlefont \@title \par}
    \vspace{1em}
    \ifx\@author\@empty\else
      {\authorfont \@author \par}
      \vspace{0.5em}
    \fi
    \ifx\@date\@empty\else
      {\datefont \@date \par}
    \fi
    \vspace{2em}
  \end{fullwidth}
}
\makeatother

% Custom abstract
\newenvironment{customabstract}{
  \begin{fullwidth}
  \begin{adjustwidth}{0.5in}{0.5in}
  \vspace{1em}
  \small
  \color{gray!30!black}
}{
  \vspace{1.5em}
  \end{adjustwidth}
  \end{fullwidth}
}



% Unicode fallback
\DeclareUnicodeCharacter{2E3B}{\textbar\textbar}

